Can Your Generative Model Detect Out-of-Distribution Covariate Shift?

Detecting Out-of-Distribution (OOD) sensory data and covariate distribution shift aims to identify new test examples with different high-level image statistics to the captured, normal and In-Distribution (ID) set. Existing OOD detection literature largely focuses on semantic shift with little-to-no consensus over covariate shift. Generative models capture the ID data in an unsupervised manner, enabling them to effectively identify samples that deviate significantly from this learned distribution, irrespective of the downstream task. In this work, we elucidate the ability of generative models to detect and quantify domain-specific covariate shift through extensive analyses that involves a variety of models. To this end, we conjecture that it is sufficient to detect most occurring sensory faults (anomalies and deviations in global signals statistics) by solely modeling high-frequency signal-dependent and independent details. We propose a novel method, CovariateFlow, for OOD detection, specifically tailored to covariate heteroscedastic high-frequency image-components using conditional Normalizing Flows (cNFs). Our results on CIFAR10 vs. CIFAR10-C and ImageNet200 vs. ImageNet200-C demonstrate the effectiveness of the method by accurately detecting OOD covariate shift. This work contributes to enhancing the fidelity of imaging systems and aiding machine learning models in OOD detection in the presence of covariate shift.

==> sections/limitations.tex <==
\section{Future Work \& Limitations}
\label{sec:limitations}

Some concerns can be raised about the complexity of the \emph{typicality} computation, since it requires a forward pass to compute the LL followed by a backpropagation computation per test sample. This increases the memory requirements when deploying the model and decreases the overall inference speed. However, in scenarios where accurate OOD covariate shift is essential, CovariateFlow provides the best accuracy vs. speed trade-offs (see Section~\ref{sec:supp_detailed_results}). 

This study did not explore the influence of the selected filter on segmenting the image into various frequency bands. Future research could delve into the impact of employing different filters and their kernel sizes, particularly when insights are available regarding the frequency bands that may harbor critical information about the covariate shift.
